Joint Debiased Representation Learning and Imbalanced Data Clustering

One of the most promising approaches for unsupervised learning is combining deep representation learning and deep clustering. Some recent works propose to simultaneously learn representation using deep neural networks and perform clustering by defining a clustering loss on top of embedded features. However, these approaches are sensitive to imbalanced data and out-of-distribution samples. As a consequence, these methods optimize clustering by pushing data close to randomly initialized cluster centers. This is problematic when the number of instances varies largely in different classes or a cluster with few samples has less chance to be assigned a good centroid. To overcome these limitations, we introduce a new unsupervised framework for joint debiased representation learning and image clustering. We simultaneously train two deep learning models, a deep representation network that captures the data distribution, and a deep clustering network that learns embedded features and performs clustering. Specifically, the clustering network and learning representation network both take advantage of our proposed statistics pooling block that represents mean, variance, and cardinality to handle the out-of-distribution samples and class imbalance. Our experiments show that using these representations, one can considerably improve results on imbalanced image clustering across a variety of image datasets. Moreover, the learned representations generalize well when transferred to the out-of-distribution dataset.

==> chapters/extra.tex <==
%---------------------------------------------------
%     Table Imbalanced CIFAR 10, CIFAR-100
%---------------------------------------------------
\begin{table*}
\centering
\caption{Comparison results of our achieved accuracy on imbalanced CIFAR-10, CIFAR-100, and MNIST.}
\label{ablation}
\begin{tabular}{l l l l l l l l l l l l }
\toprule
Dataset  & \multicolumn{4}{c}{Imbalanced CIFAR-10} &  \multicolumn{4}{c}{Imbalanced CIFAR-100} & \multicolumn{3}{c}{MNIST~\cite{lecun1998gradient}} \\
\midrule
Imbalanced Type & \multicolumn{2}{c}{long-tailed} & \multicolumn{2}{c}{step}  & \multicolumn{2}{c}{long-tailed}  & \multicolumn{2}{c}{step} & NMI & ARI & ACC  \\
\midrule
Imbalanced Ratio & 10 & 100 & 10 & 100 & 10 & 100 & 10 & 100 & & &  \\
\midrule
StatDEC  & 0.4831 & 0.4106 & {0.4872} & 0.4511 & 0.2365 & {0.1843} & 0.3716 & 0.3502 & 0.8931 & 0.8764 & 0.9343 \\
StatDEC-2  & 0.3706 & 0.3282 & 0.4306 & 0.3426 & 0.1639 & 0.1201 & 0.2363 & 0.2484 &  0.8074 & 0.7927 & 0.8526\\
StatDEC-3  & 0.4734 & 0.3887 & 0.4775 & 0.4391 & 0.2152 & 0.1678 & 0.3527 & 0.3241 &  0.8622 & 0.8445 & 0.9214\\
StatDEC+CNN  & 0.4682 & {0.4153} & 0.4818 & 0.4460 & 0.2239 & 0.1705 & 0.3704 & 0.3526 & 0.8905 & 0.8756 & 0.9368\\
StatDEC+UNet  & {0.4827} & 0.4025 & 0.4833 & 0.4838 & {0.2379} & 0.1721 & {0.3729} & {0.3480} &  0.9066 & 0.8826 & 0.9407\\
StatDEC+VAE  & 0.4536 & 0.4001 & 0.4213 & 0.4671 & 0.2291 & 0.1673 & 0.3729 & 0.3477 & 0.9041 & 0.8743 & 0.9321\\
\bottomrule
\end{tabular}
\end{table*}


\begin{figure*}[!h]
  \centering
      \subfloat[]{\includegraphics[width=0.437\textwidth]{ICCV/figures/IMBCIFAR10_ACC.png}\label{figimb_a}}
        \hfill
  \subfloat[]{\includegraphics[width=0.46\textwidth]{ICCV/figures/IMBCIFAR10_NMI.png}\label{figimb_b}}
      \hfill
  \subfloat[]{\includegraphics[width=0.42\textwidth]{ICCV/figures/cifar10.jpeg}\label{figimb_c}}
  \hfill
  \subfloat[]{\includegraphics[width=0.42\textwidth]{ICCV/figures/imbcifar10.png}\label{figimb_d}}
    \caption{Comparison of clustering performance on long-tailed imbalanced CIFAR-10 in terms of accuracy (a) and NMI (b). Visualization results of embedded clustering obtained by StatDEC-1 on step-imbalanced CIFAR-10 with a ratio of 10. (c). Visualization of deep embedded clustering on long-tailed imbalanced CIFAR-10 with a ratio of 100. (d)}
\label{fig_imb}
\end{figure*}
